RoSplat: Robust Feed-Forward Pixel-wise Gaussian Splatting for Varying Input Views and High-Resolution Rendering

Generalizable 3D Gaussian Splatting has recently emerged as an efficient approach for novel-view synthesis, enabling feed-forward synthesis from only a few input views. However, existing pixel-wise feed-forward methods suffer from over-bright renderings when the number of input views varies during inference, as well as insufficient supervision for accurate Gaussian scale estimation, which leads to hole artifacts, particularly in high-resolution renderings. To address these issues, we identify that the over-brightness is caused by the varying number of overlapping Gaussians and propose a simple alpha normalization strategy to maintain brightness consistency across different number of input views. In addition, we introduce an auxiliary 3D sampling-based regularizer to improve Gaussian scale estimation, thereby mitigating hole artifacts in high-resolution rendering. Experiments on benchmark datasets demonstrate that our method significantly improves baseline models under varying input-view and high-resolution rendering settings.

==> main/3_method_subsections/alpha_normalization_v1.tex <==

\subsection{Alpha Normalization}
\label{sub_sec:alpha_normnalization}
% How do you define number of overlapping Gaussians? 

\begin{figure}[t]
\centering
    % \setlength{\tabcolsep}{6pt}
    
    \begin{tabular}{ccc}
    \multicolumn{1}{c}{{MVSplat~\cite{}}} &
    \multicolumn{1}{c}{{TranSplat~\cite{}}} &
    \multicolumn{1}{c}{{DepthSplat~\cite{}}} \\
    
    \includegraphics[width=0.32\linewidth]{main/figures/method/alpha_norm_prev_works/0000_threeMetrics_mvsplat.jpg} &
    \includegraphics[width=0.32\linewidth]{main/figures/method/alpha_norm_prev_works/0000_threeMetrics_transplat.jpg} &
    \includegraphics[width=0.32\linewidth]{main/figures/method/alpha_norm_prev_works/0000_threeMetrics_depthsplat.jpg} \\
    \end{tabular}
    
    \caption{Your caption here.}
    \label{fig:abc_one_row}
\end{figure}

% Existing pixel-wise 3D Gaussians prediction methods often struggle to generalize to varying numbers of input views at test time. In this section, we first investigate the cause of this issue and then introduce a simple and effective alpha normalization strategy that addresses it.

Existing pixel-wise 3D Gaussians prediction methods often struggle to generalize to varying numbers of input views at test time. To better understand this phenomenon, we examine how the following three quantities produced by those works vary with the number of input views: (i) the pixel intensity of the rendered image, (ii) the accumulated compositing weight $W=\sum_j w_j(\mathbf{p})$, and (iii) the rendering quality measured by PSNR (as shown in Fig.~\ref{fig:xxx}). The figure reveals two consistent pattern. First, as input views increase, $W$ increases toward 1, which coincides with higher pixel intensity and significant drop in the image quality. Second, the magnitude of the image quality drop closely follows the change in $W$: the largest degradation occurs when $W$ increases the most (e.g., from 2 to 4 views), whereas the drop becomes less pronounced once $W$ saturates near $1.0$ (e.g., from 8 to 16 views). Together, these patterns indicate a strong correlation between the growth of the accumulated compositing weight $W$ and rendering degradation under increased input-view counts. This behavior can be attributed to the fact that increasing the number of input views typically produces more overlapping Gaussians for the same underlying 3D regions, causing more Gaussians to contribute along the same pixel ray (see the last row of Fig.~\ref{...}) and thereby increasing the accumulated compositing weight.

Consequently, these findings suggest that the over-brightness issue can be alleviated by reweighting each Gaussian's contribution based on the number of overlappings Gaussian, so as to preserve the accumulated compositing weight and improve the model's robustness to varying input-view counts. To achieve this, we adjust the alpha value $\alpha_j$ of each Gaussian used in the rendering process (see Eq.~\ref{2}) as follows: 
% \begin{equation}
%     \tilde{\alpha}_j= 1 - (1-\alpha_j)^{s_j}, \quad\quad \text{with }s_j = \min\left(1,\frac{m}{\tilde{m}_j}\right),
% \end{equation}
% \begin{equation}
% \tilde{\alpha}_j=
% \begin{cases}
% 1-(1-\alpha_j)^{\frac{m}{\tilde{m}_j}}, & \text{if } \tilde{m}_j \ge m,\\[4pt]
% \alpha_j, & \text{otherwise}.
% \end{cases}
% \end{equation}
\begin{equation}
    \tilde{\alpha}_j=1-(1-\alpha_j)^{\frac{m}{\tilde{m}_j}}
\end{equation}

where $m$ is a hyper parameter indicating the number of overlapping Gaussians corresponding to the target accumulated compositing weight we aim to preserve (e.g., $m=2$ if a model is trained with two input views) and $\tilde{m}_j$ denotes the per-Gaussian overlapping counts given the set of input views. Under the pixel-wise Gaussian prediction setting, each Gaussian's center in view $i$ is obtained by backprojecting a pixel into 3D using the predicted depth map $\mathbf{D}^{i}$, therefore the number of overlapping Gaussians $\tilde{m}_j$ can be obtained via depth consistency check. In particular, for each $i^{\text{th}}$ input view, we compute a Gaussian count map $\mathbf{\tilde{M}}^{i}\in\mathbb{R}^{H\times W}$  as follows, 
\begin{equation}
    \mathbf{\tilde{M}}^i(\mathbf{p}) = \sum_{k=1}^{K} \left\llbracket\, \frac{|\mathbf{D}^{i}(\mathbf{p}) - \mathbf{D}^{k\rightarrow i}(\mathbf{\hat{p}})|}{\mathbf{D}^{i}(\mathbf{p}) + \mathbf{D}^{k \rightarrow i}(\mathbf{\hat{p}})} \leq \tau \,\right\rrbracket
\end{equation}
with $\mathbf{\hat{p}}$ being the corresponding pixel of $\mathbf{p}$ in the $k^{\text{th}}$ input image, $\mathbf{D}^{k\rightarrow i}$ indicating the depth map of view $k$ under the same coordinate system as view $i$, $\llbracket\, \cdot \,\rrbracket$ is the Iverson bracket, and $\tau$ denotes a depth threshold value. Given $\{\mathbf{\tilde{M}}^i\}_{i=1}^K$, we can obtain a set of per-Gaussian overlapping counts $\{\tilde{m}_j\}_{j=1}^{H\times W \times K}$ which are then used for alpha normalization in Eq.~\ref{}. 

Intuitively, under an idealized case where the overlapping Gaussians are exact duplicates of each other, that is, \(W=1-\prod_{j=1}^{m}(1-\alpha)=1-(1-\alpha)^{m}\), it can be shown that \(\alpha\)-normalization preserves the same accumulated weight \(W\) when the number of duplicate Gaussians increases to \(\tilde m\): 
\begin{equation}
    \tilde W=1-(1-\tilde\alpha)^{\tilde m}=1-\Big((1-\alpha)^{m/\tilde m}\Big)^{\tilde m}=1-(1-\alpha)^m=W
\end{equation}

While a feed-forward network rarely produces perfectly duplicate Gaussians in practice, alpha normalization still stabilizes the accumulated compositing weight $W$, thereby maintaining image quality under varying numbers of input views (see dashed lines in Fig.~\ref{...}).


==> main/4_experiments_subsections/cross_dataset_generalization.tex <==

% \subsection{Cross-Dataset Evaluation}

% \noindent\textbf{Cross-Dataset Evaluation. } Here, we follow DepthSplat~\cite{xu2025depthsplat} to train our method on the RealEstate10K dataset by taking two images of resolution $256\times 448$ as inputs. We then evaluate the models on the DL3DV dataset using (1) the same configuration as training, (2) increase the number of input views to 6, (3) increase the rendering resolution to $2048\times 3584$. Tab.~\ref{tab:cross_dataset_evaluation} shows that our method retain similar performance compared to DepthSplat~\cite{xu2025depthsplat} under the same configuration used during training. On the other hand, when increasing the input views or rendering at high resolution, ours consistently outperforms DepthSplat across all metrics. This result further evident the effectiveness of our proposed alpha normalization and 3D sampling-based regularizer. 



==> main/tables/cross_dataset_eval.tex <==
% % \usepackage{color}
% % \usepackage{tabularray}
% \begin{table}
% \centering
% \footnotesize
% \begin{tblr}{
%   colsep  = 1.5pt,
%   rowsep  = 1pt,
%   column{even} = {c},
%   column{3} = {c},
%   column{5} = {c},
%   column{7} = {c},
%   column{9} = {c},
%   column{11} = {c},
%   cell{1}{2} = {c=3}{},
%   cell{1}{6} = {c=3}{},
%   cell{1}{9} = {c=3}{},
%   cell{3}{4} = {font=\bfseries},
%   cell{4}{2} = {font=\bfseries},
%   cell{4}{3} = {font=\bfseries},
%   cell{4}{6} = {font=\bfseries},
%   cell{4}{7} = {font=\bfseries},
%   cell{4}{8} = {font=\bfseries},
%   cell{4}{9} = {font=\bfseries},
%   cell{4}{10} = {font=\bfseries},
%   cell{4}{11} = {font=\bfseries},
%   vline{2-3,7,10} = {1}{},
%   vline{6} = {1}{Black},
%   vline{2,5-6,9,12} = {1-5}{Black},
%   hline{3} = {1,3,7,9-10}{Black},
%   hline{3} = {2,4,6,8,11}{},
% }
%             & 2 input views, $256 \times 448$ &        &        &   & 6 input views, $256 \times 448$ &        &        & 6 input views, $2048 \times 3584$ &        &        \\
% ~           & PSNR                    & SSIM   & LPIPS  & ~ & PSNR                     & SSIM   & LPIPS  & PSNR                         & SSIM   & LPIPS  \\
% DepthSplats & 17.50                   & 0.562  & 0.360  &   & 19.64                    & 0.670   & 0.287  & 16.80                        & 0.600   & 0.543  \\
% Ours        & 17.51                   & 0.567  & 0.362  &   & 20.64                    & 0.708  & 0.27   & 17.58                        & 0.686  & 0.521  \\
%             & +0.01                   & +0.005 & +0.002 &   & +1.00                    & +0.038 & -0.017 & +0.78                        & +0.086 & -0.022 
% \end{tblr}
% \caption{Cross-dataset evaluation. Both methods are trained on the RealEstate dataset with two input images of $256\times 448$ resolution during training. We then evaluate the models on the DL3DV dataset using (1) the same configuration as training, (2) increase the number of input views to 6, (3) Increase the rendering resolution to $2048\times 3584$ resolution.}
% \end{table}

\begin{table}[t]
\centering
\footnotesize
\caption{\textbf{Cross-dataset evaluation}. Both methods are trained on the RealEstate dataset with two input images of $256\times 448$ resolution. We evaluate the models on the DL3DV dataset using (1) the same configuration as training, (2) increase the number of input views to 6, (3) increase the rendering resolution to $2048\times 3584$ resolution.}
% \resizebox{\textwidth}{!}{
\begin{tblr}{
  colsep  = 1.5pt,
  rowsep  = 1pt,
  % 1 left-aligned column for methods, 9 fixed-width centered columns for metrics
  colspec = {l *{9}{Q[c, wd=4em]}}, 
  % Define column spans for the group headers
  cell{1}{2} = {c=3}{c},
  cell{1}{5} = {c=3}{c},
  cell{1}{8} = {c=3}{c},
  % Solid vertical lines to separate the method column and the three main groups
  vline{2,5,8} = {solid},
  % Solid horizontal lines for clean structure
  hline{3,5} = {solid},   % Top border, under headers, and bottom border
  % hline{2} = {1-10}{solid}, % Border exactly underneath the view count headers
}
& 2 views, $256 \times 448$ & & & 6 views, $256 \times 448$ & & & 6 views, $2048 \times 3584$ & & \\

& PSNR $\uparrow$  & SSIM $\uparrow$  & LPIPS $\downarrow$ & PSNR $\uparrow$  & SSIM $\uparrow$  & LPIPS $\downarrow$ & PSNR $\uparrow$  & SSIM $\uparrow$ & LPIPS $\downarrow$\\

DepthSplat & 17.50 & 0.562 & \textbf{0.360} & 19.64 & 0.670 & 0.287 & 16.80 & 0.600 & 0.543 \\

Ours & \textbf{17.51} & \textbf{0.567} & 0.362 & \textbf{20.64} & \textbf{0.708} & \textbf{0.27} & \textbf{17.58} & \textbf{0.686} & \textbf{0.521} \\

& \textcolor{Green}{+0.01} & \textcolor{Green}{+0.005} & \textcolor{orange}{+0.002} & \textcolor{Green}{+1.00} & \textcolor{Green}{+0.038} & \textcolor{Green}{-0.017} & \textcolor{Green}{+0.78} & \textcolor{Green}{+0.086} & \textcolor{Green}{-0.022} \\
\end{tblr}
% }
\label{tab:cross_dataset_evaluation}
\end{table}

==> supps/cross_dataset_evaluation.tex <==

\section{Cross-dataset Evaluation}
For cross-dataset evaluation, we follow DepthSplat~\cite{xu2025depthsplat} to train our method on the RealEstate10K dataset by taking two images of resolution $256\times 448$ as inputs. We then evaluate the models on the DL3DV dataset using (1) the same configuration as training, (2) increase the number of input views to 6, (3) increase the rendering resolution to $2048\times 3584$. Tab.~\ref{tab:cross_dataset_evaluation} shows that our method retain similar performance compared to DepthSplat~\cite{xu2025depthsplat} under the same configuration used during training. On the other hand, our method demonstrates superiority when evaluated under test settings that differ from training. Specifically, when increasing the input views or rendering at high resolution, our method consistently achieve better image quality across all metrics compared to DepthSplat. This result further evidents the effectiveness of our proposed alpha normalization and 3D sampling-based regularizer. 


==> supps/figures/alpha_norm_curve.tex <==

\begin{figure}[t]
\centering
    % \setlength{\tabcolsep}{6pt}
    
    \begin{tabular}{ccc}
    \multicolumn{1}{c}{{MVSplat~\cite{chen2024mvsplat}}} &
    \multicolumn{1}{c}{{TranSplat~\cite{zhang2025transplat}}} &
    \multicolumn{1}{c}{{DepthSplat~\cite{xu2025depthsplat}}} \\
    
    \includegraphics[width=0.32\linewidth]{supps/Figures/alpha_norm_curve/31b8eb8bbebed9b8_threeMetrics_mvsplat.jpg} &
    \includegraphics[width=0.32\linewidth]{supps/Figures/alpha_norm_curve/31b8eb8bbebed9b8_threeMetrics_transplat.jpg} &
    \includegraphics[width=0.32\linewidth]{supps/Figures/alpha_norm_curve/31b8eb8bbebed9b8_threeMetrics_depthsplat.jpg} \\
    \end{tabular}
    
    \caption{Pixel intensity, accumulated compositing weight, image quality (PSNR), and number of predicted Gaussians under varying input-view counts. \textbf{First row}: Median gray-scale pixel intensity across the whole image. \textbf{Second row}: Median total accumulated weight across the whole image. \textbf{Third row}: Image quality measured via PSNR. \textbf{Last row}: Median number of Gaussians used for rendering. To compute this, we first obtain the number of Gaussians involve in the rendering process for each pixel, then compute the median value across all pixels. \textbf{Analysis}: Increasing the number of input views causes existing feed-forward Gaussian Splatting methods~\cite{chen2024mvsplat, zhang2025transplat, xu2025depthsplat} to predict more overlapping Gaussians (last row), which increases the accumulated compositing weight $W$ (second row), raises pixel intensity (first row), leading to overbright images and PSNR degradation (third row). Our alpha normalization mitigates this effect by stabilizing $W$, leading to more consistent brightness and improved rendering quality.}
    \label{fig:alpha_norm_curve}
\end{figure}

==> supps/figures/alpha_norm_vis_1.tex <==

\begin{figure}
\centering
\footnotesize

\begin{tblr}[]{
  width = 0.95\linewidth,
  colsep = 1pt,
  rowsep = 0.0pt, % Set explicitly to 0pt
  stretch = 0.25,  % Turns off default line stretching
  row{2-Z} = {abovesep=0pt, belowsep=0pt}, % Kills inner cell padding for all image rows
  colspec = {Q[wd=4mm,c,m] X[c,m] X[c,m] X[c,m] X[c,m]},
  row{1} = {abovesep=2pt, belowsep=2pt}, % Keeps a normal gap for your text header
  cell{1-Z}{1} = {halign=c, valign=m}, 
  % hline{5} = {dashed, abovesep=0pt, belowsep=0pt},
}

 & 2 views & 4 views & 8 views & 16 views \\

% \smash{\rotatebox[origin=c]{90}{2 views}} &  
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/mvsplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/depthsplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/transplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/gt.png} \\

\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{Ground-truth}}} &  
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/gt.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{DepthSplat~\cite{xu2025depthsplat}}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_2views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_4views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_8views_FalseAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_16views_FalseAlpha.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\SetRow{abovesep=2pt}
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{\cite{xu2025depthsplat} + $\alpha$ norm.}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_2views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_4views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_8views_TrueAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/09b505bb829c1d12/depthsplat_rendered_16views_TrueAlpha.jpg} \\

\hline[dashed, wd=0.5pt] 
\SetRow{belowsep=4pt}

\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{Ground-truth}}} &  
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/gt.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{TranSplat~\cite{zhang2025transplat}}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_2views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_4views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_8views_FalseAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_16views_FalseAlpha.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{\cite{zhang2025transplat} + $\alpha$ norm.}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_2views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_4views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_8views_TrueAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/308de3d523189c72/transplat_rendered_16views_TrueAlpha.jpg}

\end{tblr}
\caption{\textbf{Qualitative results on RealEstate10K dataset}. Here, we apply alpha normalization to existing works~\cite{zhang2025transplat, xu2025depthsplat} \textbf{without retraining}. Prior methods~\cite{zhang2025transplat, xu2025depthsplat} encounter overbrightness issue when the number of input views is greater than two. Integrating alpha normalization ($\alpha$ norm.)
helps to mitigate their overbrightness issues when increasing the number of input views. }
\label{fig:qualitative_result_alpha_norm_1}
\end{figure}

==> supps/figures/alpha_norm_vis_2.tex <==

\begin{figure}
\centering
\footnotesize

\begin{tblr}[]{
  width = 0.95\linewidth,
  colsep = 1pt,
  rowsep = 0.0pt, % Set explicitly to 0pt
  stretch = 0.25,  % Turns off default line stretching
  row{2-Z} = {abovesep=0pt, belowsep=0pt}, % Kills inner cell padding for all image rows
  colspec = {Q[wd=4mm,c,m] X[c,m] X[c,m] X[c,m] X[c,m]},
  row{1} = {abovesep=2pt, belowsep=2pt}, % Keeps a normal gap for your text header
  cell{1-Z}{1} = {halign=c, valign=m}, 
  % hline{5} = {dashed, abovesep=0pt, belowsep=0pt},
}

 & 2 views & 4 views & 8 views & 16 views \\

% \smash{\rotatebox[origin=c]{90}{2 views}} &  
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/mvsplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/depthsplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/transplat_rendered_2views_TrueAlpha.png} &
% \includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/gt.png} \\

\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{Ground-truth}}} &  
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/gt.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{MVSplat~\cite{chen2024mvsplat}}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_2views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_4views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_8views_FalseAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_16views_FalseAlpha.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\SetRow{abovesep=2pt}
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{\cite{chen2024mvsplat} + $\alpha$ norm.}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_2views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_4views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_8views_TrueAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/28742766eb882cd2/mvsplat_rendered_16views_TrueAlpha.jpg} \\

\hline[dashed, wd=0.5pt] 
\SetRow{belowsep=4pt}

\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{Ground-truth}}} &  
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/gt.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/gt.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{TranSplat~\cite{zhang2025transplat}}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_2views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_4views_FalseAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_8views_FalseAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_16views_FalseAlpha.jpg} \\

% --- REMOVED BLANK LINES HERE ---
\raisebox{35pt}{\smash{\rotatebox[origin=c]{90}{\cite{zhang2025transplat} + $\alpha$ norm.}}} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_2views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_4views_TrueAlpha.jpg} &
\includegraphics[width=\linewidth]{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_8views_TrueAlpha.jpg} & 
\includegraphics[width=\linewidth]
{supps/Figures/alpha_norm_vis/e07392b123f6fd77/transplat_rendered_16views_TrueAlpha.jpg}

\end{tblr}
\caption{\textbf{Qualitative results on RealEstate10K dataset}. Here, we apply alpha normalization to existing works~\cite{zhang2025transplat, chen2024mvsplat} \textbf{without retraining}. Prior methods~\cite{zhang2025transplat, chen2024mvsplat} encounter overbrightness issue when the number of input views is greater than two. Integrating alpha normalization ($\alpha$ norm.)
helps to mitigate their overbrightness issues when increasing the number of input views. }
\label{fig:qualitative_result_alpha_norm_2}
\end{figure}

==> supps/figures/depth_sensitivity.tex <==



\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{supps/Figures/metrics_vs_depth_threshold.jpg}
    \caption{\textbf{Sensitivity to depth error threshold}. Using a threshold of 0.5 results in the best image quality across all metrics.}
    \label{fig:depth_sensitivity}
\end{figure}



==> supps/figures/gaussians.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.78\textwidth]{main/Figures/hole_scenes/hole-scenes-v2.png}
    \caption{\textbf{Gaussians visualizations on the DL3DV dataset}. We can see that scenes reconstructed by DepthSplat~\cite{xu2025depthsplat} show many hole artifacts in zoom-in views, while ours shows few or even no hole artifacts (white cracked areas in above figures).}
    \label{fig:gaussian_visualization}
\end{figure}


==> supps/figures/high_resolution_vis.tex <==


\begin{figure}
    \centering
    % Set to 0pt if you want absolutely no gap between the images
    \setlength{\tabcolsep}{1pt} 
    
    \begin{tabular}{ccc}
        % --- Header Row ---
        Ground-truth & DepthSplat~\cite{xu2025depthsplat} & Ours \\


        % --- Row 1 Images ---
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0017_9e9a89ae6fed06d6e2f4749b4b0059f35ca97f848cedc4a14345999e746f7884/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0017_9e9a89ae6fed06d6e2f4749b4b0059f35ca97f848cedc4a14345999e746f7884/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0017_9e9a89ae6fed06d6e2f4749b4b0059f35ca97f848cedc4a14345999e746f7884/ours.jpg} \\


        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0011_5c3af581028068a3c402c7cbe16ecf9471ddf2897c34ab634b7b1b6cf81aba00/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0011_5c3af581028068a3c402c7cbe16ecf9471ddf2897c34ab634b7b1b6cf81aba00/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0011_5c3af581028068a3c402c7cbe16ecf9471ddf2897c34ab634b7b1b6cf81aba00/ours.jpg} \\
        
        
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0018_8fdc5130f0731360cc053f59049bfe6db509567457c5471c970292966cb34f17/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0018_8fdc5130f0731360cc053f59049bfe6db509567457c5471c970292966cb34f17/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0018_8fdc5130f0731360cc053f59049bfe6db509567457c5471c970292966cb34f17/ours.jpg} \\

        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0013_c076929db6501cf7ebe386c70e6d77ea3af844a745e794f2ec17c981c465a69b/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0013_c076929db6501cf7ebe386c70e6d77ea3af844a745e794f2ec17c981c465a69b/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0013_c076929db6501cf7ebe386c70e6d77ea3af844a745e794f2ec17c981c465a69b/ours.jpg} \\

        % --- Row 2 Images ---
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0015_ba55c875d20c34ee85ffc72264c4d77710852e5fb7d9ce4b9c26a8442850e98f/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0015_ba55c875d20c34ee85ffc72264c4d77710852e5fb7d9ce4b9c26a8442850e98f/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0015_ba55c875d20c34ee85ffc72264c4d77710852e5fb7d9ce4b9c26a8442850e98f/ours.jpg} \\
        
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0012_adf35184a12d4cfa3f4248b87aa5adb4f39f179df460d6d76136e13d37299a2a/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0012_adf35184a12d4cfa3f4248b87aa5adb4f39f179df460d6d76136e13d37299a2a/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0012_adf35184a12d4cfa3f4248b87aa5adb4f39f179df460d6d76136e13d37299a2a/ours.jpg} \\

        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0019_f477ffc4b398bed8e0d921f0fba9825ca63f317381c535c84be23be991ae1d7a/gt.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0019_f477ffc4b398bed8e0d921f0fba9825ca63f317381c535c84be23be991ae1d7a/depth_splat.jpg} & 
        \includegraphics[width=0.32\linewidth]{supps/Figures/high_resolution_vis_compress/3840x2160/0019_f477ffc4b398bed8e0d921f0fba9825ca63f317381c535c84be23be991ae1d7a/ours.jpg} \\
        
    \end{tabular}
    
    \caption{\textbf{High-resolution rendering on DL3DV dataset}. Our method significantly alleviates the holes issues exhibited by DepthSplat~\cite{xu2025depthsplat}. }
    \label{fig:qualitative_result_high_resolution}
\end{figure}


==> supps/more_analysis.tex <==


\section{More Analysis on the Over-Brightness Issue}
\label{sec:more_analysis_overbrightness}

To provide further evidence for the over-brightness analysis in the main paper, examine how the following three quantities produced by existing works~\cite{chen2024mvsplat, zhang2025transplat, xu2025depthsplat} vary with the number of input views: (i) the pixel intensity of the rendered image, (ii) the accumulated compositing weight $W=\sum_j w_j(\mathbf{p})$, and (iii) the rendering quality measured by PSNR. Specifically, for each method and input-view count in Fig.~\ref{fig:alpha_norm_curve}, we compute pixel-wise statistics on a rendered target image and summarize them using the median over all pixels. For the first row in the figure, we convert the rendered image to grayscale, then compute the median grayscale intensity. We then evaluate the accumulated compositing weight at each pixel as $W(\mathbf p)=\sum_j w_j(\mathbf p)$, and report its median value across all pixels (second row). PSNR is computed between the rendered image and the ground-truth target image (third row). Finally, we count the number of Gaussians contributing to each pixel and report the median count (fourth row). 

The figure reveals a consistent pattern across all three methods. As the number of input views increases, the number of contributing Gaussians also increases (last row of Fig.~\ref{fig:alpha_norm_curve}), indicating that more Gaussians overlap on the same underlying scene regions. This increase in overlap is accompanied by a monotonic increase in the accumulated compositing weight $W$ (second row of Fig.~\ref{fig:alpha_norm_curve}), leading to a monotonic increase in the pixel intensity (first row of Fig.~\ref{fig:alpha_norm_curve}), a degradation in the image quality~(third row of Fig.~\ref{fig:alpha_norm_curve}). Moreover, the largest PSNR drop is consistently observed when the increase in $W$ is the most pronounced, while the degradation becomes less severe once $W$ saturates near $1$. These observations provide strong empirical support for the analysis in the main paper (Sec. 4.1): the over-brightness issue mainly arises because increasing the number of input views produces more overlapping Gaussians, which increases the accumulated compositing weight and leads to degraded rendering quality.

In contrast, after applying our alpha normalization, the accumulated compositing weight remains much more stable across different input-view counts. As a result, the rendered pixel intensity also stays more consistent, and the rendering quality is significantly improved compared to without alpha normalization. This demonstrates that stabilizing the accumulated compositing weight is an effective way to mitigate the over-brightness issue and improve robustness under varying input-view counts.

\input{main/tables/cross_dataset_eval}
\input{supps/tables/zoomin_evaluation}
\input{supps/figures/alpha_norm_curve}

\section{Sensitivity to Depth Error Threshold}
\input{supps/figures/depth_sensitivity}
Fig~\ref{fig:depth_sensitivity} show the performance of our method with different depth error thresholds. The plot reveals that setting the threshold to 0.5 shows the best performance across all metrics. On the other hand, threshold higher than 0.5 lead to minor drop in the image quality, while thresholds below 0.5 result in higher degradation.  





==> supps/more_qualitative_result_alpha_norm.tex <==

\section{More Qualitative Results}
Fig.~\ref{fig:gaussian_visualization} visualizes the Gaussians predicted by our method and DepthSplat. It shows that our method produces Gaussians with larger scales, leading to better coverage of the 3D scene. In contrast, DepthSplat~\cite{xu2025depthsplat} tends to predict overly small-scale Gaussians, which results in hole artifacts.

In Figs.~\ref{fig:qualitative_result_alpha_norm_1} and \ref{fig:qualitative_result_alpha_norm_2}, we provide additional qualitative comparisons to show the effect of applying alpha normalization to existing methods~\cite{chen2024mvsplat, zhang2025transplat, xu2025depthsplat}. Moreover, Fig.~\ref{fig:qualitative_result_high_resolution} presents further visual comparisons between our method and DepthSplat~\cite{xu2025depthsplat} for high-resolution rendering. The results show that our method mitigates the over-brightness and hole artifacts exhibited by existing methods. 

\input{supps/figures/gaussians}

\input{supps/figures/alpha_norm_vis_1}
\input{supps/figures/alpha_norm_vis_2}
\input{supps/figures/high_resolution_vis}





==> supps/tables/zoomin_evaluation.tex <==

% \usepackage{color}
% \usepackage{tabularray}

\begin{table}[t]
\centering
\scriptsize
\caption{\textbf{Comparison on the DL3DV dataset under zoom-in rendering}. Our method significantly outperforms DepthSplat, and the performance gaps increases as the zoom-in factor increases.}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  colsep  = 1.5pt,
  rowsep  = 1pt,
  column{even} = {c},
  column{3} = {c},
  column{5} = {c},
  column{7} = {c},
  column{9} = {c},
  column{11} = {c},
  column{13} = {c},
  cell{1}{2} = {c=3}{},
  cell{1}{6} = {c=3}{},
  cell{1}{9} = {c=3}{},
  cell{1}{12} = {c=3}{},
  cell{3}{2} = {font=\bfseries},
  cell{3}{3} = {font=\bfseries},
  cell{3}{4} = {font=\bfseries},
  cell{4}{6} = {font=\bfseries},
  cell{4}{7} = {font=\bfseries},
  cell{4}{8} = {font=\bfseries},
  cell{4}{9} = {font=\bfseries},
  cell{4}{10} = {font=\bfseries},
  cell{4}{11} = {font=\bfseries},
  cell{4}{12} = {font=\bfseries},
  cell{4}{13} = {font=\bfseries},
  cell{4}{14} = {font=\bfseries},
  vline{2} = {1}{Black},
  vline{3,6-7,10,13} = {1}{},
  vline{2,5-6,9,12} = {1-5}{Black},
  hline{3} = {1,4,6,8,11,14}{},
  hline{3} = {2-3,7,9-10,12-13}{Black},
  hline{5} = {1,4,6,8,11,14}{},
  hline{5} = {2-3,7,9-10,12-13}{Black}
}
           & $1\times$ zoom-in &        &       &   & $2\times$ zoom-in  &       &        & $4\times$ zoom-in  &       &        & $8\times$ zoom-in  &       &        \\
           & PSNR $\uparrow$        & SSIM $\uparrow$  & LPIPS $\downarrow$ & ~ & PSNR $\uparrow$           & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$            & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$           & SSIM $\uparrow$  & LPIPS  $\downarrow$  \\
DepthSplat & 24.17 & 0.819 & 0.145 & & 19.95 & 0.676 & 0.272 & 17.05 & 0.528 & 0.436 & 16.07 & 0.512 & 0.511  \\
Ours        & 24.10 & 0.818 & 0.147 & & 20.84 & 0.692 & 0.263 & 18.79 & 0.587 & 0.398 & \textbf{18.19} & \textbf{0.586} & \textbf{0.477}  \\
~           & \textcolor{orange}{-0.07} & \textcolor{orange}{-0.001} & \textcolor{orange}{+0.002} & & \textcolor{Green}{+0.89} & \textcolor{Green}{+0.016} & \textcolor{Green}{-0.009} & \textcolor{Green}{+1.74} & \textcolor{Green}{+0.059} & \textcolor{Green}{-0.038} & \textcolor{Green}{+2.12} & \textcolor{Green}{+0.074} & \textcolor{Green}{-0.034} 
\end{tblr}
}
\label{tab:zoomed_in_comparision}
\end{table}

==> supps/zoom_in_evaluation.tex <==



\section{Zoom-in Rendering}
Tab.~\ref{tab:zoomed_in_comparision} compares our method with DepthSplat under centered zoom-in rendering. Specifically, we render zoomed-in images by multiplying the focal length by the zoom factor while keeping the principal point fixed at the image center. All zoomed-in images are rendered at the training resolution of $256\times 448$. To construct the corresponding ground-truth images, we center-crop high-resolution images so that they match the same zoom factor. For example, the ground-truth image for $8\times$ zoom-in is obtained by center-cropping the corresponding $8\times$ higher-resolution ground-truth image to a resolution of $256\times 448$. Tab.~\ref{tab:zoomed_in_comparision} shows that our method achieves better image quality than DepthSplat under zoom-in rendering. Moreover, the performance gap increases as the zoom factor increases. These results further demonstrate the effectiveness of our 3D sampling-based strategy for improving Gaussian scale estimation.


